Learning Identifiable Gaussian Bayesian Networks in Polynomial Time and Sample Complexity

Learning the directed acyclic graph (DAG) structure of a Bayesian network from observational data is a notoriously difficult problem for which many hardness results are known. In this paper we propose a provably polynomial-time algorithm for learning sparse Gaussian Bayesian networks with equal noise variance --- a class of Bayesian networks for which the DAG structure can be uniquely identified from observational data --- under high-dimensional settings. We show that $O(k^4 \log p)$ number of samples suffices for our method to recover the true DAG structure with high probability, where $p$ is the number of variables and $k$ is the maximum Markov blanket size. We obtain our theoretical guarantees under a condition called Restricted Strong Adjacency Faithfulness, which is strictly weaker than strong faithfulness --- a condition that other methods based on conditional independence testing need for their success. The sample complexity of our method matches the information-theoretic limits in terms of the dependence on $p$. We show that our method out-performs existing state-of-the-art methods for learning Gaussian Bayesian networks in terms of recovering the true DAG structure while being comparable in speed to heuristic methods.

==> estimating_reg_coeffs_old.tex <==
\subsection{Estimating regression coefficients}
The conditional distribution of $X_i$ given all the remaining variables is given as:
$X_i | X_{\mi} = \vx \sim \mathcal{N}(\vth_i^T \vx,\, \nicefrac{1}{\Omega_{i,i}})$,
which leads to the following generative model for $\mX_{*,i}$:
\begin{align}
\mX_{*,i} = (\mX_{*, \mi}) \vth^*_i + \veps'_i, \label{eq:gen_model_lasso}
\end{align}
where $\veps'_i \simiid \mathcal{N}(0, \nicefrac{1}{\Omega_{i,i}})$ and 
$\mX_{j, \mi} \simiid \mathcal{N}(\vect{0}, \mSig_{\mi, \mi})$
for all $j \in [n]$.
Therefore, for all $i \in [p]$, we obtain the estimator $\vhth_i$ for $\vth^*_i$ by solving the following
$\ell_1$-constrained least squares problem:
\begin{align}
\vhth_i = \argmin_{\vbeta \in \R^{(p - 1)}} \NormII{\mX_{*,i} - (\mX_{*,\mi}) \vbeta}^2 + \lambda \NormI{\vbeta}. \label{eq:lasso}
\end{align}
The above optimization problem, which goes by the name of \emph{Lasso}, has been extensively
analyzed in the statistics and compressed sensing literature; 
necessary and sufficient conditions for its success are fairly well understood. 
We invoke the results of Wainwright \cite{wainwright_sharp_2009}
to derive our main result in this sub-section.

\begin{lemma}
Let $(\G, \Pf(\Ws, \sigma^2))$ be a GBN with $\mSig^*$ and $\mtOmg$ being the covariance and inverse covariance
matrix over $X$. Let $\vhth_i$ be the solution to \eqref{eq:gen_model_lasso} 
obtained by solving \eqref{eq:lasso}. Under Assumptions \ref{ass:faithfulness}, \ref{ass:nonsingular} and \ref{ass:incoherence}, and
if the regularization parameter and number of samples satisfy:
\begin{gather*}
\sqrt{\frac{4 (\max_{j \in \Ss^c_i \setminus \Set{i}} \Sigma^*_{j,j})}{\Omega^*_{i,i} \cmin \gamma^2} \frac{\log p}{n}} <
\lambda_n \leq  \Bigl(\nicefrac{1}{\NormInfty{\mSig_{\Ss_i, \Ss_i}^{-\nicefrac{1}{2}}}} \Bigr)
	\biggl(\frac{\alpha}{\sigma^2 \Omega^*_{i,i}} - 20 \sqrt{\cramped{\frac{\log k}{n \cmin \Omega^*_{i,i}}}} \biggr), \\
n > \frac{2 (\max_{j \in \Ss^c_i \setminus \Set{i}} \Sigma^*_{j,j}) }{\cmin \gamma^2} (k \log (p - k)),
\end{gather*}
then $\NormInfty{\vhth_i - \vth^*_i} \leq \nicefrac{\alpha}{\sigma^2 \Omega^*_{i,i}}$, with probability
at least $1 - c_1 \exp(c_2 \min\{k, \log(p -k)\})$, where $c_1, c_2 > 0$ are constants
and $\Ss_i \defeq \Sp(\vth^*_i)$ and $|\Ss_i| \leq k$.
\end{lemma}

%First note that, from the characterization of $\vth_i$ in Lemma \ref{lemma:theta},
%we have: $\Sp(\vth_i) \subseteq \MB_i$. Let $\Abs{\MB_i} \defeq k_i$.
\begin{proof}
We first show that Assumption \ref{ass:incoherence} implies the mutual incoherence condition of Wainwright \cite{wainwright_sharp_2009}.
Denote $\mtlSig \defeq \mSig^*_{\mi, \mi}$ and $\mtlOmg \defeq (\mSig^*_{\mi, \mi})^{-1} = 
\mtOmg_{\mi, \mi} - \mtOmg_{-i, i} (\mtOmg_{i, i})^{-1} \mtOmg_{i, -i}$.
The incoherence condition as defined by Wainwright is: $\NormInfty{\mtlSig_{\Ss_i^c,\Ss_i} (\mtlSig_{\Ss_i,\Ss_i})^{-1}} \leq 1 - \gamma$.
Observe that $\NB_i \subseteq \Ss_i \subseteq \MB_i$. We use a stronger version of incoherence, for reasons which will become clear later,
and require that $\NormInfty{\mtlSig_{\NB_i^c,\NB_i} (\mtlSig_{\NB_i,\NB_i})^{-1}} \leq 1 - \gamma$. 
For the purpose of this proof we will not include the node $i$ in the set $\NB_i^c$.
The incoherence condition is then given as:
\begin{align}
\NormInfty{\mtlSig_{\NB_i^c,\NB_i} (\mtlSig_{\NB_i,\NB_i})^{-1}} &=
	\max_{j \in \NB_i^c} \NormI{\mtlSig_{j,\NB_i} (\mtlSig_{\NB_i,\NB_i})^{-1}}  \label{eq:inc1}
\end{align}
Fix any $j \in \NB_i^c$, and denote by $\mbrSig$ and $\mbrOmg$ the covariance and precision matrix, respectively,
over the set $X_{\Set{j} \union \NB_i}$. Then we have
\begin{align}
\mtlSig_{j,\NB_i} (\mtlSig_{\NB_i,\NB_i})^{-1} = 
	\mbrSig_{j,\NB_i} (\mbrSig_{\NB_i,\NB_i})^{-1} =
	 - \frac{\mbrOmg_{u,\NB_i}}{\bar{\Omega}_{u,u}}, \label{eq:inc2}
\end{align}
where the last equality is a standard result for Gaussians. Combining \eqref{eq:inc1} and \eqref{eq:inc2} we get
Assumption \ref{ass:incoherence}.

From Theorem 3 of \cite{wainwright_sharp_2009} the constant $\theta_u(\mSig^*)$, defined in \cite{wainwright_sharp_2009},
is bounded as follows:
\begin{align*}
\theta_u(\mSig^*) \leq \frac{1}{\cmin \gamma^2} 
	\Bigl(\max_{j \in \Ss^c_i \setminus \Set{i}} \Sigma^*_{j,j} - \mSig^*_{j,\Ss_i} (\mSig^*_{\Ss_i, \Ss_i})^{-1} \mSig^*_{\Ss_i, j} \Bigr)
	\leq \frac{\max_{j \in \Ss^c_i \setminus \Set{i}} \Sigma^*_{j,j}}{\cmin \gamma^2}.
\end{align*}
Note that the true regression parameter satisfies, for $j \in \Ss_i$, 
$\Abs{\vth^*_{i,j}} = \nicefrac{\Abs{\Omega^*_{i,j}}}{\Omega^*_{i,i}} \geq \nicefrac{3 \alpha}{\sigma^2 \Omega^*_{i,i}}$,
by Assumption \ref{ass:faithfulness}.
Therefore, we need to have $\NormInfty{\vhth_i - \vth^*_i} \leq \nicefrac{\alpha}{\sigma^2 \Omega^*_{i,i}}$ in order
to ensure correct support recovery. This implies, from Theorem 3 of \cite{wainwright_sharp_2009}, the following
upper bound on the regularization parameter:
\begin{align*}
\lambda_n \leq \Bigl(\nicefrac{1}{\NormInfty{\mSig_{\Ss_i, \Ss_i}^{-\nicefrac{1}{2}}}} \Bigr)
	\biggl(\frac{\alpha}{\sigma^2 \Omega^*_{i,i}} - 20 \sqrt{\cramped{\frac{\log k}{n \cmin \Omega^*_{i,i}}}} \biggr).
\end{align*}
Since, $\lambda_n > 0$, this requires that $\alpha > 20 \sigma^2 \sqrt{\cramped{\frac{(\Omega^*_{i,i}) \log k}{n \cmin }}}$.
The lower bound on $\lambda_n$ and the number of samples comes directly from Theorem 3 of Wainwright \cite{wainwright_sharp_2009}.
\end{proof}
